Dynamic Connected Cooperative Coverage Problem

We study the so-called dynamic coverage problem by agents located in some topological graph. The agents must visit all regions of interest but they also should stay connected to the base via multi-hop. We prove that the algorithmic complexity of this planning problem is PSPACE-complete. Furthermore we prove that the problem becomes NP-complete for bounded plans. We also prove the same complexities for the reachability problem of some positions. We also prove that complexities are maintained for a subclass of topological graphs.

==> section_discussion.tex <==
\subsection{Battery}
\todo{on gère les batteries}


\subsection{Constraints}
\todo{objectif plus compliqué : LTL ?}


==> section_modelchecking.tex <==
\newcommand{\codegeek}{\textsf}
\subsection{Tests}
We implemented a tool to solve \problemcoverage with two methods: model checking and planning. Indeed, both techniques deal with Kripke structures (also called transition systems) and can express reachability goals (here ``the graph is covered and all UAVs are back at the base''). The model checking part is done with the model checker NuSMV \cite{cimatti2000nusmv}, which is a classical symbolic model checker for Linear Temporal Logic (LTL \cite{pnueli1977temporal}).  The planning part is done with classical planning and is expressed in the Planning Domain Description Language \cite{mcdermott1998pddl}. We use the planner FS (for Functional STRIPS), as it is shown to have similar time complexities in respect to current best classical planners \cite{DBLP:conf/ijcai/FrancesRLG17}. Furthermore, FS allows to specify values of some predicates or functions in an external C file, avoiding tedious descriptions of some sophisticated predicates in propositional logic. In our case, for instance, an external C function tests the connectivity of the UAV subgraph (active communications in Figure \ref{figure:exampleexecution}). 
% The tool is available on the following url:
%\begin{center}
%	\url{http://people.irisa.fr/Francois.Schwarzentruber/dronestrategy/}
%\end{center}
%as well as a GUI that displays the generated covering executions.
%Here, we handle battery level constraints: each UAV $i$ has a battery level, noted $b(i)$, initially at max value $b_{max}$, that decreases by one unit each time $i$ is not at $B$, and increases to $b_{max}$ when $i$ is at $B$.

\newcommand{\drone}{i}
\newcommand{\droneb}{j}
\newcommand{\node}{v}



\begin{figure}[t]

		
	\centering
	\scalebox{0.8}{\begin{tabular}{c}
		Undirected neighbor-communicable graphs with $n = |V|$: \\	
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		$|V|$ & Mc yes &  no & To & FS yes & no &  To \\
		\hline
		5 & \textbf{68 (0.14 s)} & \textbf{32 (1.1 s)} & 0 & 68 (3.1 s) & 22 (74.2 s) & 10 \\
		\hline
		10 & \textbf{98 (2.1 s)} & \textbf{2 (16.8 s)} & 0 & 98 (5.0 s) & 0 & 2 \\
		\hline
		15 & 83 (19.0 s) & 0 & 17 & \textbf{100 (8.8 s)} & 0 & 0 \\
		\hline
		20 & 55 (55.8 s) & 0 & 45 & \textbf{100 (26.4 s)} & 0 & 0 \\
		\hline
	\end{tabular} \\

	Undirected neighbor-communicable graphs with $n = |V|/2$: \\
		
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		$|V|$ & Mc yes &  no & To & FS yes & no &  To \\
		\hline
		5 & \textbf{63 (0.04 s)} & \textbf{37 (0.2 s)} & 0 & 63 (1.6 s) & 37 (1.4 s) & 0 \\
		\hline
		10 & \textbf{99 (0.34 s)} & \textbf{1 (2.8 s)} & 0 & 99 (0.98 s) & 0 & 1 \\
		\hline
		15 & 99 (1.7 s) & 0 & 1 & \textbf{100 (1.3 s)} & 0 & 0 \\
		\hline
		20 & 61 (24.2 s) & 0 & 39 & \textbf{100 (4.3 s)} & 0 & 0 \\
		\hline
	\end{tabular}\\

	Arbitrary graphs with $n = |V|$: \\
	
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		$|V|$ & Mc yes &  no & To & FS yes & no &  To \\
		\hline
		5 & \textbf{28 (0.14 s)} & \textbf{72 (1.4 s)} & 0 & 28 (0.5 s) & 47 (24.2 s) & 25 \\
		\hline
		10 & 85 (2.1 s) & \textbf{13 (43.02 s)} & 2 & \textbf{85 (1.3 s)} & 2 (3.0 s) & 13 \\
		\hline
		15 & 95 (11.8 s) & \textbf{2 (158.6 s)} & 3 & \textbf{96 (4.6 s)} & 0 & 4 \\
		\hline
		20 & 96 (55.8 s) & 0 & 4 & \textbf{98 (19.7 s)} & 0 & 2 \\
		\hline
	\end{tabular}\\
	
	Arbitrary graphs with $n = |V|/2$: \\
	
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		$|V|$ & Mc yes &  no & To & FS yes & no &  To \\
		\hline
		5 & \textbf{14 (0.03 s)} & \textbf{86 (0.21 s)} & 0 & 14 (0.44 s) & 86 (0.54 s) & 0 \\
		\hline
		10 & \textbf{83 (0.32 s)} & \textbf{17 (3.4 s)} & 0 & 83 (1.3 s) & 8 (0.48 s) & 9 \\
		\hline
		15 & 99 (1.2 s) & 1 (17.5 s) & 0 &\textbf{ 99 (1.0 s)} & \textbf{1 (7.4 s)} & 0 \\
		\hline
		20 & 95 (5.2 s) & \textbf{1 (266.4 s)} & 4 & \textbf{99 (3.6 s)} & 0 & 1 \\
		\hline
	\end{tabular}
	\end{tabular}}
	
	\caption{Experimental results \label{figure:results}}
\end{figure}

To test both implementations, we perform randomly generated tests. The tests depend on the number UAVs $n$ and on the number of nodes of the topological graph $|V|$. 
%The max battery level is always $3|V|$ to focus only on the existence of a coverage in the tests.  
 We distinguish two classes of topologic graphs:
 \begin{itemize}
 	\item Undirected neighbor-communicable graphs, who may appear more often in practical applications.
 	\item Arbitrary graphs, which may be directed and not include neighbor communications, to test the methods with unconstrained graphs. 
 \end{itemize}  Furthermore we distinguish two possible values for $n$: 
 \begin{itemize}
 	\item $n = |V|$ for an extreme case where there is as much UAVs as nodes. I this case, the search of the solution is independent of the number of UAVs, so we just search whether it is possible to cover the graph independently from the number of UAVs.
 	\item $n = |V|/2$, which is a central case where it is not sufficient to fill the graph with UAVs to find a solution.
 \end{itemize}
 Altogether four types of tests are defined. The results are displayed in Figure~\ref{figure:results}.
%\begin{itemize}
%	\item Undirected neighbor-communicable graphs:
%	\begin{itemize}
%		\item Case where $n = m$ with $b_{max} = 3m$: a case which rarely fails (Figure \ref{figure:fullsym}). 
%		\item Case where $n = m/2$ with $b_{max} = 3m$: a more sophisticated case (Figure \ref{figure:halfsym}).
%	\end{itemize}
%	\item Completely random graphs:
%	\begin{itemize}
%		\item Case where $n = m$ with $b_{max} = 3m$ (Figure \ref{figure:fullnotsym}).
%		\item Case where $n = m/2$ with $b_{max} = 3m$ (Figure \ref{figure:halfnotsym}).
%	\end{itemize}
%\end{itemize}
%The problem \problemcoverage is fairly new, so no suitable test yet exist. These four categories of tests capture for graphs close to reality (undirected and neighbor-communicable graphs) and random graphs in a almost-always feasible case which is $n = m$ and a harder case where $n = m/2$.

\subsection{Results}
We run 100 tests for each type of test on a HP EliteBook 840 G2 with a timeout of 300 seconds. The ``yes'' columns refer to the number of tests in which a plan was found, with the mean time in parentheses. The ``no'' columns refer to the number of tests in which the solver returned that no plan exists. The ``To'' column refer to the number of tests that resulted in a timeout. In each table, the first column corresponds to $|V|$, the following three are the results for model checking and the last three are the results for planning. The best results between NuSMV and FS are written in bold text.

The criteria for evaluating which of the two is best, in the ``yes'' or ``no'' columns, is the number of tests that succeeded. For instance in the the third table, case $|V| = 10$, NuSMV found that no solution existed for 13 tests whereas FS found that no solution existed for 2 cases. It means that although FS was better for these two cases, it got a timeout for 11 other tests where no solution should have been found. Therefore, we estimate here that NuSMV was better even though the mean time was worse. If both NuSMV and FS find the same number in any column, the mean time is considered to evaluate which one is the best. 


NuSMV is globally better for a small number of nodes (typically $|V| \leq 10$). The reason is that FS has an incompressible preprocessing time, so for small instances, the preprocessing time is higher that the actual solving time.

For bigger instances, FS is better than NuSMV for the ``yes'' cases, i.e. the solvable instances. For the unsolvable instances, NuSMV tends to be better but there are few unsolvable instances to validate this result. Indeed, it is hard to conceive unsolvable instances that are not obvious (like two disconnected components), so the random generation creates much more solvable instances that unsolvable ones.

 Furthermore, arbitrary graphs are easier than undirected neighbor-communicable graphs because each transition in an undirected graph is represented by two directed transitions. Thus, an undirected graph has usually more possible transitions than a directed graph, so the search space is bigger. In the same way, even though it seems easier to find a solution when $n = |V|$, the search space includes the position of each UAV so it is bigger when $n = |V|$. Therefore, the mean times for $n = |V|/2$ are smaller than the mean times for $n = |V|$.  
 
 Altogether, FS is better than NuSMV. Yet, for as far as we know, it is worthwhile to consider NuSMV because it is easier to implement extensions compared to planners. Indeed, model checking deals with infinite traces, where it is possible to express properties as ``The UAVs visit infinitely often the nodes''. In planning, only reachability properties can be express of the form ``in the future it is true that \dots''.  %Yet, NuSMV has the advantage of being flexible, because adding new constraints consists in adding new atoms in the model and changing the goal formula. 

%\todo{phrase introductive qui explique ce qu'on raconte là... mais... quid de mettre ça plutôt dans la conclusion ?}
%In FS, the model itself must be changed to add new constraints\todo{donner les exemples des contraintes ICI}, including the preconditions and effects of the actions, which amounts to starting from scratch\todo{starting from scratch what???}. Furthermore\todo{On the contrary?}, NuSMV allows more expressive property than planning, as ``visit all nodes infinitely often'' or ``use all UAVs infinitely often'' that are defined on infinite executions, which is not possible in FS where only reachability properties can be expressed on finite executions.   
%Full sym:
%
%\begin{tabular}{|c|c|c|c|c|c|c|}
%	\hline
%	n= & SMV found & SMV not found & SMV timeout & Plan found & Plan not found & Plan timeout \\
%	\hline
%	4 & 63 (0.07) & 37 (0.44) & 0 & 63 (0.5) & 37 (0.89) & 0 \\
%	\hline
%	5 & 68 (0.14) & 32 (1.1) & 0 & 68 (3.1) & 22 (74.2) & 10 \\
%	\hline
%	6 & 81 (0.3) & 19 (2.0) & 0 & 81 (4.4) & 8 (16.0) & 11 \\
%	\hline
%	7 & 90 (0.47) & 10 (3.7) & 0 & 90 (4.7) & 2 (5.4) & 8 \\
%	\hline
%	8 & 92 (0.88) & 8 (5.2) & 0 & 92 (4.7) & 2 (5.4) & 5 \\
%	\hline
%	9 & 96 (1.3) & 4 (10.5) & 0 & 96 (4.9) & 0 & 4 \\
%	\hline
%	10 & 98 (2.1) & 2 (16.8) & 0 & 98 (5.0) & 0 & 2 \\
%	\hline
%	11 & 98 (3.5) & 2 (24.1) & 0 & 98 (5.3) & 0 & 1 \\
%	\hline
%	12 & 99 (9.8) & 1 (31.7) & 0 & 99 (5.9) & 0 & 0 \\
%	\hline
%	13 & 100 (17.0) & 0 & 0 & 100 (6.7) & 0 & 0 \\
%	\hline
%	14 & 80 (27.5) & 0 & 20 & 100 (7.7) & 0 & 0 \\
%	\hline
%	15 & 83 (19.0) & 0 & 17 & 100 (8.8) & 0 & 0 \\
%	\hline
%	16 & 70 (23.2) & 0 & 28 & 99 (10.6) & 0 & 0 \\
%	\hline
%	17 & 73 (26.7) & 0 & 27 & 100 (14.9) & 0 & 0 \\
%	\hline
%	18 & 63 (32.9) & 0 & 37 & 100 (18.5) & 0 & 0 \\
%	\hline
%	19 & 73 (40.2) & 0 & 27 & 100 (23.8) & 0 & 0 \\
%	\hline
%	20 & 55 (55.8) & 0 & 45 & 100 (26.4) & 0 & 0 \\
%	\hline
%\end{tabular}
%
%Half sym:
%
%\begin{tabular}{|c|c|c|c|c|c|c|}
%	\hline
%	n= & SMV found & SMV not found & SMV timeout & Plan found & Plan not found & Plan timeout \\
%	\hline
%	4 & 63 (0.03) & 37 (0.14) & 0 & 63 (2.1) & 37 (1.4) & 0 \\
%	\hline
%	5 & 63 (0.04) & 37 (0.2) & 0 & 63 (1.6) & 37 (1.4) & 0 \\
%	\hline
%	6 & 81 (0.08) & 19 (0.45) & 0 & 81 (1.2) & 19 (25.9) & 0 \\
%	\hline
%	7 & 92 (0.09) & 8 (0.55) & 0 & 92 (1.1) & 5 (134.1) & 2 \\
%	\hline
%	8 & 93 (0.17) & 8 (1.9) & 0 & 93 (1.0) & 0 & 6 \\
%	\hline
%	9 & 99 (0.2) & 1 (1.2) & 0 & 99 (0.98) & 0 & 0 \\
%	\hline
%	10 & 99 (0.34) & 2 (2.8) & 0 & 99 (0.98) & 0 & 0 \\
%	\hline
%	11 & 99 (0.37) & 1 (2.6) & 0 & 99 (0.92) & 0 & 0 \\
%	\hline
%	12 & 100 (0.93) & 0 & 0 & 100 (0.99) & 0 & 0 \\
%	\hline
%	13 & 100 (0.75) & 0 & 0 & 100 (0.99) & 0 & 0 \\
%	\hline
%	14 & 100 (5.5) & 0 & 0 & 100 (1.2) & 0 & 0 \\
%	\hline
%	15 & 99 (1.7) & 0 & 0 & 100 (1.3) & 0 & 0 \\
%	\hline
%	16 & 98 (20.4) & 1 (18.2) & 0 & 99 (1.7) & 0 & 0 \\
%	\hline
%	17 & 95 (17.6) & 0 & 4 & 100 (1.8) & 0 & 0 \\
%	\hline
%	18 & 78 (19.0) & 0 & 22 & 100 (2.8) & 0 & 0 \\
%	\hline
%	19 & 89 (25.5) & 0 & 11 & 100 (3.1) & 0 & 0 \\
%	\hline
%	20 & 61 (24.2) & 0 & 39 & 100 (4.3) & 0 & 0 \\
%	\hline
%\end{tabular}
%
%Full not sym:
%
%\begin{tabular}{|c|c|c|c|c|c|c|}
%	\hline
%	n= & SMV found & SMV not found & SMV timeout & Plan found & Plan not found & Plan timeout \\
%	\hline
%	4 & 19 (0.06) & 81 (0.5) & 0 & 19 (0.48) & 81 (3.5) & 0 \\
%	\hline
%	5 & 28 (0.14) & 72 (1.4) & 0 & 28 (0.5) & 47 (24.2) & 25 \\
%	\hline
%	6 & 26 (0.25) & 74 (3.3) & 0 & 26 (0.5) & 36 (12.1) & 38 \\
%	\hline
%	7 & 55 (0.46) & 45 (7.4) & 0 & 55 (3.9) & 23 (5.2) & 22 \\
%	\hline
%	8 & 71 (0.71) & 29 (12.5) & 0 & 71 (0.91) & 12 (5.7) & 17 \\
%	\hline
%	9 & 74 (1.2) & 25 (30.6) & 0 & 74 (1.5) & 6 (48.5) & 20 \\
%	\hline
%	10 & 85 (2.1) & 0 & 2 & 85 (1.3) & 2 (3.0) & 13 \\
%	\hline
%	11 & 89 (2.8) & 8 (64.0) & 2 & 89 (1.9) & 2 (9.5) & 8 \\
%	\hline
%	12 & 94 (4.1) & 5 (88.2) & 0 & 94 (2.9) & 1 (63.5) & 5 \\
%	\hline
%	13 & 96 (6.4) & 3 (114.4) & 0 & 96 (4.0) & 0 & 3 \\
%	\hline
%	14 & 98 (10.4) & 0 & 1 & 99 (3.2) & 0 & 0 \\
%	\hline
%	15 & 95 (11.8) & 2 (158.6) & 3 & 96 (4.6) & 0 & 3 \\
%	\hline
%	16 & 95 (16.5) & 1 (277.5) & 3 & 95 (5.9) & 0 & 5 \\
%	\hline
%	17 & 95 (23.7) & 0 & 5 & 100 (7.8) & 0 & 0 \\
%	\hline
%	18 & 96 (37.0) & 0 & 4 & 98 (10.1) & 0 & 2 \\
%	\hline
%	19 & 93 (44.4) & 0 & 6 & 100 (14.0) & 0 & 0 \\
%	\hline
%	20 & 96 (55.8) & 0 & 4 & 98 (19.7) & 0 & 2 \\
%	\hline
%\end{tabular}
%
%Half not sym:
%
%\begin{tabular}{|c|c|c|c|c|c|c|}
%	\hline
%	n= & SMV found & SMV not found & SMV timeout & Plan found & Plan not found & Plan timeout \\
%	\hline
%	4 & 13 (0.03) & 87 (0.15) & 0 & 13 (0.52) & 87 (0.51) & 0 \\
%	\hline
%	5 & 14 (0.03) & 86 (0.21) & 0 & 14 (0.44) & 86 (0.54) & 0 \\
%	\hline
%	6 & 33 (0.07) & 67 (0.61) & 0 & 33 (0.47) & 67 (36.8) & 0 \\
%	\hline
%	7 & 41 (0.09) & 59 (0.92) & 0 & 41 (0.47) & 42 (75.0) & 17 \\
%	\hline
%	8 & 67 (0.17) & 33 (6.9) & 0 & 67 (0.51) & 13 (0.46) & 20 \\
%	\hline
%	9 & 76 (0.2) & 24 (2.4) & 0 & 76 (0.61) & 5 (0.72) & 19 \\
%	\hline
%	10 & 83 (0.32) & 17 (3.4) & 0 & 83 (1.3) & 8 (0.48) & 9 \\
%	\hline
%	11 & 90 (0.37) & 10 (4.6) & 0 & 90 (1.5) & 6 (0.57) & 3 \\
%	\hline
%	12 & 96 (0.6) & 4 (10.0) & 0 & 96 (0.71) & 2 (0.59) & 1 \\
%	\hline
%	13 & 97 (0.72) & 3 (16.6) & 0 & 97 (0.72) & 1 (8.9) & 1 \\
%	\hline
%	14 & 97 (1.1) & 3 (30.9) & 0 & 97 (1.0) & 2 (6.4) & 0 \\
%	\hline
%	15 & 99 (1.2) & 1 (17.5) & 0 & 99 (1.0) & 1 (7.4) & 0 \\
%	\hline
%	16 & 97 (2.4) & 3 (78.6) & 0 & 97 (1.4) & 2 (101.1) & 1 \\
%	\hline
%	17 & 96 (2.4) & 4 (146.4) & 0 & 96 (1.7) & 0 & 3 \\
%	\hline
%	18 & 95 (3.6) & 2 (95.9) & 3 & 97 (2.0) & 1 (3.7) & 1 \\
%	\hline
%	19 & 93 (8.0) & 5 (148.3) & 1 & 95 (2.3) & 1 (32.0) & 4 \\
%	\hline
%	20 & 95 (5.2) & 1 (266.4) & 4 & 99 (3.6) & 0 & 0 \\
%	\hline
%\end{tabular}
%We use LTL bounded model checking on some examples. LTL (unbounded) model checking and CTL model checking were inefficient. We furthermore added battery level constraints, that have been modeled straightforwardly: a fixed and finite number of levels of batteries for each UAVs, each UAV loses one level of battery level at each transition, each UAV recharges its battery level when going to the base.
%
%
%The following table gives an idea of the running time:

%\begin{center}
%\begin{tabular}{l|l|l}
%\#UAVs & \#level of batteries & Execution time \\
%\hline
%3 & 12 &	3m52.408s \\
%3 & 20 & 4m51.609s \\
%4 & 12 & 38m18.751s \\
%4 & 100 & 5m14.156s \\
%4 & 20 & 8m3.822s \\
%3 & - & 3m51.694s
%\end{tabular}
%\end{center}
